Metric Renormalization in General Relativity

The averaging problem in general relativity concerns the difficulty of defining meaningful averages of tensor quantities and we consider various aspects of the problem. We first address cosmological backreaction which arises because the averaged Einstein tensor is not the same as the Einstein tensor of the averaged metric. It has been suggested that backreaction might account for the dark energy. We show numerically in the Buchert formalism that the corrections from (quasi)linear perturbations are only of the order of 10^-5 and act as a dark matter. We then focus on constructing averaged metrics and present a generally covariant averaging process which decomposes the metric into Vielbeins and parallel transports them with a relativistic Wegner-Wilson operator to a single point where they can then be averaged. The Vielbeins are chosen in a Lagrangian formalism. The functionality of the process is demonstrated in specific examples in two and three space dimensions. This involves the numerical solution of partial differential equations by the aid of the simulation toolkit Gascoigne.

==> format.tex <==
\newcommand{\del}{\partial}
\newcommand{\be}{\begin{equation}\begin{aligned}}
\newcommand{\ee}{\end{aligned}\end{equation}}
\newcommand{\D}{\displaystyle}
\newcommand{\arccot}{\operatorname{arccot}}
\newcommand{\arctanh}{\operatorname{arctanh}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\av}[1]{\left< #1\right>}
\newcommand{\intdom}[1]{\frac{1}{V}\int_{\mathcal{D}} #1\sqrt{h}d^3\mathbf{x}}
\newcommand{\dom}[1]{#1_{\mathcal{D}}}
\newcommand{\Qd}{\mathcal{Q}_{\mathcal{D}}}
\newcommand{\Rd}{\mathcal{R}_{\mathcal{D}}}
\newcommand{\Pd}{\mathcal{P}_{\mathcal{D}}}
\newcommand{\Td}{\mathcal{T}_{\mathcal{D}}}
\newcommand{\bkr}{\overline{\rho}}


==> ricciflow.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{The Ricci Flow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

